Evaluating Cognitive Age Alignment in Interactive AI Agents

While agentic AI and its core multimodal large language models (MLLMs) have demonstrated remarkable promise in language and visual reasoning across domains ranging from daily life to advanced scientific research, a profound gap remains between artificial and human intelligence. Despite the integration of powerful tools and advanced MLLMs, state-of-the-art AI agents frequently fail at foundational, seemingly simple tasks that a child can resolve with ease. Inspired by the Wechsler Intelligence Scale for Children (WISC), we introduce ChildAgentEval, the first psychometrically grounded interactive benchmark for evaluating cognitive age alignment in MLLM-based agents. ChildAgentEval systematically compares the reasoning performance of various MLLM-based interactive agents against age-specific human developmental stages, exposing where current agentic AI systems can and cannot simulate age-specific cognitive behavior.

==> sec/1_intro.tex <==
\section{Introduction}


Large Language Models (LLMs) and their derivative agentic systems have fundamentally transformed human-AI interaction. By leveraging sophisticated tool-use, strategic planning, and vast knowledge bases, these agents now assist humans across diverse domains, including education~\citep{kasneci2023chatgpt}, healthcare~\citep{Zhang2023.07.10.23292373, singhal2023large}, scientific research~\citep{boiko2023emergent, chen2025mlrbench}, and daily productivity \citep{luo2025largelanguagemodelagent}. To date, these agentic evaluations have predominantly followed a performance-maximization paradigm: assessing whether an agent can solve increasingly complex tasks to match or surpass adult expert performance~\citep{phan2025humanity,lu2022learn}. However, as agents evolve from transient tools into long-term interactive partners, a critical yet overlooked question emerges: \emph{Can an agent's capabilities be reliably calibrated to a specific cognitive profile, rather than merely maximized?}

This challenge is particularly salient for AI systems deployed in pediatric and adolescent contexts. Middle childhood and early adolescence represent critical developmental windows characterized by rapid cognitive shifts and identity formation~\citep{eccles1999development}. Current AI-driven tutors, companion robots, and mental health supports frequently engage with users across these distinct developmental stages~\citep{murali2026evaluatingllmsafetychild, nayeem2024kidlmadvancinglanguagemodels, liu2025benchmarkingllmsmimickingchildcaregiver}. In such scenarios, technical correctness is insufficient. An agent that relies exclusively on adult-level abstractions and complex reasoning may transcend a child's cognitive limits, failing to identify specific points of confusion or providing guidance that is developmentally mismatched. For child-facing AI, the primary objective shifts from raw problem-solving power to cognitive simulation: the ability to align its communicative and reasoning style with the developmental state of its partner.

Children are not low-scoring adults in intelligence. Developmental psychology shows systematic changes across age in vocabulary abstraction, working memory capacity, visual spatial reasoning, hypothesis testing, processing speed, attention control, and social perspective taking. Younger children rely more on concrete experience and visual salience \citep{piaget1952origins}, have shorter memory spans\citep{Cowan2010Magical, Gathercole1999CognitiveAT}, and are more easily misled by surface features. With age, children gradually develop abstract categorization, rule induction, multi step reasoning, counterfactual thinking, and more general social understanding. Therefore, a developmentally aligned agent should not simply use simpler language or intentionally answer fewer items correctly. It should show age matched patterns in reasoning strategy, memory capacity, attention bias, language form, and errors. Existing agent evaluations and LLM benchmarks do not answer this question. They can show whether a model is strong in problem solving, but they do not show whether it has age specific cognitive structure under developmental psychology and clinical psychometrics. What is missing is a paradigm for evaluating and controlling \emph{cognitive age alignment}: whether an agent can show the cognitive ability, language features, and error patterns of a target child age in interactive tasks for age-specific users.

In this work, we investigate developmental calibration: whether an AI agent can align its cognitive profile to a specific target age. To evaluate this, we adopt a clinical psychometric framework. While standard AI benchmarks measure task success, they lack the theoretical foundation for age-specific cognition. Clinical tests provide validated normative data, distinct cognitive factors, and standardized protocols, enabling objective measurement against grounded developmental baselines rather than subjective assumptions. Therefore, we introduce \benchmarknamec, an interactive framework inspired by the Wechsler Intelligence Scale for Children (WISC-IV) \citep{wechsler2003wisc}.  Instead of reproducing protected clinical items, ChildAgentEval draws on the WISC-IV framework, ensuring that its web-based tasks are informed by the target cognitive constructs that cover verbal comprehension, perceptual and fluid reasoning, working memory. Offline agents click, select, and navigate within a live browser under realistic constraints like time limits. Performance analysis was assisted by a professional WISC-IV assessor. To move beyond simplistic role-prompting, we further propose a Data-Grounded Skill Distillation strategy with the evaluation pipeline. This approach extracts developmental indicators from empirical pediatric data into structured ``cognitive skill cards'', injecting them as executable constraints on the agent's language, memory, and reasoning. Experiments on multimodal agents demonstrate that while standard prompting yields flat trajectories, our distillation method facilitates robust age differentiation.
Our work makes four main contributions:
\begin{enumerate}[label=(\arabic*), leftmargin=*,itemsep=0.5ex, parsep=0pt, topsep=0pt]
\item We define \textbf{cognitive age alignment} as a novel challenge, shifting the evaluation focus from maximizing raw capability to calibrating agent behaviors against human developmental structures.
\item We build {\benchmarkname}, a WISC-inspired interactive web evaluation pipeline supporting age-based administration, dynamic stopping rules, and granular behavioral logging.
\item We introduce a data-driven \textbf{Skill Distillation} strategy that transforms empirical developmental traits into executable constraints for agents.
\item We empirically demonstrate that standard prompting fails to produce stable developmental trajectories, whereas our distillation strategy significantly improves age differentiation and reveals current LLM limitations in calibrating working memory and visuospatial reasoning.
\end{enumerate}

% Overall, ChildAgentBench is not intended to assign a simple intelligence score to an AI agent. It provides a framework that connects developmental psychology with agent behavior evaluation, and studies a more basic question: when AI agents enter human developmental environments, can they not only become more capable, but also reason, explain, remember, and make errors in ways that are appropriate for a given age.







==> sec/related_works.tex <==
\section{Related Work}
% \vspace{-1mm}
% Our work is closely related to Psychometric and Cognitive Evaluation of LLMs and MLLMs, LLMs as Cognitive Models and Human Simulators, and Child-focused LLM Simulation and Safety. A comprehensive discussion is provided in Appendix \ref{sec:relatedwork}

% Our work intersects with three emerging areas of artificial intelligence evaluation. First, regarding the psychometric and cognitive evaluation of large language models, recent studies have begun adapting adult-oriented intelligence tests and population-normed benchmarks to assess foundation models~\citep{hao2025visuallargelanguagemodels, galatzer2024cognitive}. Second, researchers increasingly utilize language models as cognitive simulators and agentic proxies for human behavior~\citep{binz2025centaurfoundationmodelhuman, xie2024largelanguagemodelagents}. Third, child-focused AI research has primarily concentrated on aligning model safety protocols and linguistic styles for younger users~\citep{murali2026evaluatingllmsafetychild, nayeem2024kidlmadvancinglanguagemodels}. 

% Our work intersects three research areas: (1) psychometric evaluation via adult-oriented benchmarks \citep{hao2025visuallargelanguagemodels,galatzer2024cognitive, ahrabian2024nonverbal,qu2024integration,li2026toward}; (2) the use of LLMs as cognitive simulators and human proxies \citep{binz2025centaurfoundationmodelhuman, xie2024largelanguagemodelagents, li2025reflectionbench, sartori2023psychological}; and (3) child-facing AI safety and style alignment \citep{murali2026evaluatingllmsafetychild, nayeem2024kidlmadvancinglanguagemodels}.
% However, existing literature lacks a framework to measure whether an agent truly reasons like a specific age group. Our work distinguishes itself by shifting the focus from static evaluation to interactive developmental calibration. A comprehensive discussion is provided in Appendix~\ref{sec:relatedwork}. \looseness-1

